Type Ia supernovae in NS+He star systems and the isolated mildly recycled pulsars

Type Ia supernovae (SNe Ia) are successful cosmological distance indicators and important element factories in the chemical evolution of galaxies. They are generally thought to originate from thermonuclear explosions of carbon-oxygen white dwarfs in close binaries. However, the observed diversity among SNe Ia implies that they have different progenitor models. In this article, we performed the long-term evolution of NS+He star binaries with different initial He star masses ($M_{\rm He}^{\rm i}$) and orbital periods ($P_{\rm orb}^{\rm i}$) for the first time, in which the He star companions can explode as SNe Ia eventually. Our simulations indicate that after the He stars develop highly degenerate oxygen-neon (ONe) cores with masses near the Chandrasekhar limit, explosive oxygen burning can be triggered due to the convective Urca process. According to these calculations, we obtained an initial parameter space for the production of SNe Ia in the $\rm log\,$$P^{\rm i}_{\rm orb}-M^{\rm i}_{\rm He}$ plane. Meanwhile, we found that isolated mildly recycled pulsars can be formed after He stars explode as SNe Ia in NS+He star binaries, in which the isolated pulsars have minimum spin periods ($P_{\rm spin}^{\rm min}$) of $\sim 30-110\rm\,ms$ and final orbital velocities of $\sim \rm 60-360\,km\,s^{-1}$, corresponding to initial orbital periods of $0.07-10\rm\,d$. Our work suggests that the NS+He star channel may contribute to the formation of isolated mildly recycled pulsars with velocity $\rm \lesssim 360\,km\,s^{-1}$ in observations, and such isolated pulsars should locate in the region of pulsars with massive WD companions in the $P_{\rm spin}-\dot P_{\rm spin}$ diagram.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

